The Future of HCI-Policy Collaboration

Policies significantly shape computation's societal impact, a crucial HCI concern. However, challenges persist when HCI professionals attempt to integrate policy into their work or affect policy outcomes. Prior research considered these challenges at the ``border'' of HCI and policy. This paper asks: What if HCI considers policy integral to its intellectual concerns, placing system-people-policy interaction not at the border but nearer the center of HCI research, practice, and education? What if HCI fosters a mosaic of methods and knowledge contributions that blend system, human, and policy expertise in various ways, just like HCI has done with blending system and human expertise? We present this re-imagined HCI-policy relationship as a provocation and highlight its usefulness: It spotlights previously overlooked system-people-policy interaction work in HCI. It unveils new opportunities for HCI's futuring, empirical, and design projects. It allows HCI to coordinate its diverse policy engagements, enhancing its collective impact on policy outcomes.

==> discussion.tex <==
% % policy is the ``\textit{broader impact}'' of HCI's human understanding and tech design contributions~\cite{HCI-policy-boundary-CHI19} rather than a distinctive intellectual contribution itself.

==> figure_av.tex <==

\begin{figure*}[h]
    \includegraphics[width=0.9\textwidth]{figures/rw_interactions_taller-cropped-full.pdf}

    \captionsetup{width=0.9\textwidth}
  \caption{Mapping the many ways driverless vehicles' behaviors, service design, urban design, and law and policy influence each other. They offer each other both design opportunities (green arrows) and constraints (red arrows).}
  \Description{A diagram mapping the many ways driverless vehicles' motion design, service design, urban design, and law and policy influence each other. They offer each other both new opportunities (green arrows) and constraints (red arrows).}
%   \vspace{0.2cm}
\label{fig:interactions}
\end{figure*}  


==> table_policyQs.tex <==
\begin{table*}[ht]
    \centering
    \renewcommand{\arraystretch}{1.2} 
    \begin{tabularx}{1\textwidth}{X l l}
        \toprule[2pt]
        \textbf{\shortstack{Questions\\Raised}} & \textbf{\shortstack{Relevant\\Policy Concepts}} & \textbf{\shortstack{Example Answers\\from Policy and Related Literature}} \\
        
        \addlinespace[1mm]
        \hline
        \addlinespace[1mm]
        
        How can tech and policy design dismantle oppressive systems? 
        & Theory of Change & Policy is the art of incremental change. \\
        
        
        \bottomrule[2pt]
    \end{tabularx}
    % \captionsetup{width=0.95\linewidth}
    \vspace{0.2cm}
    \caption{\qian{Policy questions. These questions come out of discussions~\TODOcite, but for anonymity, we put the questions without references.}}
    \label{tab:policyQs}
    %\vspace{-3em}
\end{table*}
